Near-Optimal No-Regret Learning for Correlated Equilibria in Multi-Player General-Sum Games

Recently, Daskalakis, Fishelson, and Golowich (DFG) (NeurIPS`21) showed that if all agents in a multi-player general-sum normal-form game employ Optimistic Multiplicative Weights Update (OMWU), the external regret of every player is $O(\textrm{polylog}(T))$ after $T$ repetitions of the game. We extend their result from external regret to internal regret and swap regret, thereby establishing uncoupled learning dynamics that converge to an approximate correlated equilibrium at the rate of $\tilde{O}(T^{-1})$. This substantially improves over the prior best rate of convergence for correlated equilibria of $O(T^{-3/4})$ due to Chen and Peng (NeurIPS`20), and it is optimal -- within the no-regret framework -- up to polylogarithmic factors in $T$. To obtain these results, we develop new techniques for establishing higher-order smoothness for learning dynamics involving fixed point operations. Specifically, we establish that the no-internal-regret learning dynamics of Stoltz and Lugosi (Mach Learn`05) are equivalently simulated by no-external-regret dynamics on a combinatorial space. This allows us to trade the computation of the stationary distribution on a polynomial-sized Markov chain for a (much more well-behaved) linear transformation on an exponential-sized set, enabling us to leverage similar techniques as DFG to near-optimally bound the internal regret. Moreover, we establish an $O(\textrm{polylog}(T))$ no-swap-regret bound for the classic algorithm of Blum and Mansour (BM) (JMLR`07). We do so by introducing a technique based on the Cauchy Integral Formula that circumvents the more limited combinatorial arguments of DFG. In addition to shedding clarity on the near-optimal regret guarantees of BM, our arguments provide insights into the various ways in which the techniques by DFG can be extended and leveraged in the analysis of more involved learning algorithms.

==> figs/UNUSED_trees_3nodes.tex <==
\begin{comment}
\begin{figure}
    \centering
    \begin{tikzpicture}[
        roundnode/.style={circle, draw=black!100, fill=white!5, thick, minimum size=8mm},
        rootnode/.style={circle, draw=black!100, fill=white!5, very thick, minimum size=8mm},
        ]
        %Nodes
        \node[rootnode]      (1)                              {1};
        \node[roundnode]    (2)       [below left=of 1] {2};
        \node[roundnode]      (3)       [below right=of 1] {3};
        
        %Lines
        \draw[->, line width=.3mm] (2) -- (1);
        \draw[->, line width=.3mm] (3) -- (1);
    \end{tikzpicture}
    \hspace{15mm}
    \begin{tikzpicture}[
        roundnode/.style={circle, draw=black!100, fill=white!5, thick, minimum size=8mm},
        rootnode/.style={circle, draw=black!100, fill=white!5, very thick, minimum size=8mm},
        ]
        %Nodes
        \node[rootnode]      (1)                              {1};
        \node[roundnode]      (3)       [below=of 1] {3};
        \node[roundnode]    (2)       [right=of 3] {2};
        
        
        %Lines
        \draw[->, line width=.3mm] (2) -- (1);
        \draw[->, line width=.3mm] (3) -- (2);
    \end{tikzpicture}
    \hspace{15mm}
    \begin{tikzpicture}[
        roundnode/.style={circle, draw=black!100, fill=white!5, thick, minimum size=8mm},
        rootnode/.style={circle, draw=black!100, fill=white!5, very thick, minimum size=8mm},
        ]
        %Nodes
        \node[rootnode]      (1)                              {1};
        \node[roundnode]    (2)       [below=of 1] {2};
        \node[roundnode]      (3)       [right=of 2] {3};
        
        %Lines
        \draw[->, line width=.3mm] (3) -- (1);
        \draw[->, line width=.3mm] (2) -- (3);
    \end{tikzpicture}
    \caption{All the possible $3$-node directed trees rooted at node $1$.}
    \label{fig:directed_trees}
\end{figure}
\end{comment}

==> text/proofs.tex <==

\section{Omitted Proofs from \texorpdfstring{\Cref{section:main}}{Section 3}}
\label{appendix:proofs-3}

In this section we provide all of the missing proofs from \cref{section:external_regret}. We commence with the proof of \cref{lemma:high-order-smooth}. For the convenience of the reader, the statement of the lemma is included below.

\highsmooth*

\begin{proof}[Proof of \cref{lemma:high-order-smooth}]
First of all, we know that 
\begin{equation}
    \label{eq:utility-game}
    \vec{\ell}_i^{(t)}[a_i] = \sum_{a_{i'} \in \range{n_{i'}}, i' \neq i} \Lambda(a_1, \dots, a_i, \dots, a_m) \prod_{i' \neq i} \vec{x}^{(t)}_{i'}[a_{i'}],
\end{equation}
where recall that by assumption $\Lambda(\cdot) \in [0,1]$. In particular, given that $\vec{L}^{(t)}_{i}[\edge{j}{k}] = \vec{x}^{(t)}_i[j](\vec{\ell}^{(t)}_i[k] - \vec{\ell}^{(t)}_i[j])$, we may conclude that 
\begin{equation}
    \label{eq:L-loss}
    \vec{L}_i^{(t)}[\edge{j}{k}] = \sum_{a_{i'} \in \range{n_{i'}}, i' \neq i} \mleft( \Lambda(a_1, \dots, k, \dots, a_m) - \Lambda(a_1, \dots, j, \dots, a_m) \mright) \vec{x}^{(t)}_i[j] \prod_{i' \neq i} \vec{x}^{(t)}_{i'}[a_{i'}].
\end{equation}
However, we know from the equivalence shown in \cref{theorem:equivalence} that $\vec{x}_{i'}^{(t)}[a_{i'}] = \sum_{\tree_{i'} \in \treeset_{i', a_{i'}}} \vec{X}_{i'}^{(t)}[\tree_{i'}]$. Given that the set of directed trees with different roots are disjoint, \eqref{eq:L-loss} can be expressed as
\begin{equation}
    \label{eq:LX-loss}
    \vec{L}_i^{(t)}[\edge{j}{k}] = \sum_{\tree_{i'} \in \treeset_{i'}} \Lambda'(\tree_{1}, \dots, \tree_m) \prod_{i' \in \range{m}} \vec{X}^{(t)}_{i'}[\tree_{i'}],
\end{equation}
where $\Lambda': \treeset_1 \times \dots \times \treeset_m \to [-1, 1]$. In particular, this implies that 
\begin{align}
    \left\lvert (D_h \vec{L}_i)^{(t)}[\edge{j}{k}] \right\rvert &= \left\lvert \sum_{s=0}^h \binom{h}{s} (-1)^{h - s} \vec{L}_i^{(t + s)}[\edge{j}{k}] \right\rvert \label{eq:align-binom} \\
    &= \left\lvert \sum_{\tree_{i'} \in \treeset_{i'}} \Lambda'(\tree_1, \dots, \tree_m) \sum_{s=0}^h \binom{h}{s} (-1)^{h - s} \prod_{i' \in \range{m}} \vec{X}^{(t+s)}_{i'}[\tree_{i'}] \right\rvert \label{eq:align-Lloss} \\
    &\leq \sum_{\tree_{i'} \in \treeset_{i'}} \left\lvert  \sum_{s=0}^h \binom{h}{s} (-1)^{h - s} \prod_{i' \in \range{m}} \vec{X}^{(t+s)}_{i'}[\tree_{i'}] \right\rvert \label{eq:align-triangle} \\
    &= \sum_{\tree_{i'} \in \treeset_{i'}} \left\lvert \mleft( D_h \mleft( \prod_{i' \in \range{m}} \vec{X}_{i'}[\tree_{i'}] \mright) \mright)^{(t)} \right\rvert \label{eq:bound-Li},
\end{align}
where \eqref{eq:align-binom} uses the equivalent formulation \eqref{eq:binomial} of $h$-order finite differences; \eqref{eq:align-Lloss} follows from \eqref{eq:LX-loss}; \eqref{eq:align-triangle} follows from the triangle inequality and the fact that $|\Lambda'(\cdot)| \in [0, 1]$; and the final line uses again the equivalent formulation of finite differences of \eqref{eq:binomial}, with the convention that $\prod_{i' \in \range{m}} \vec{X}_{i'}[\tree_{i'}]$ refers to the sequence $\prod_{i' \in \range{m}} \vec{X}^{(1)}_{i'}[\tree_{i'}], \dots, \prod_{i' \in \range{m}} \vec{X}^{(T)}_{i'}[\tree_{i'}]$. Next, it will be convenient to assume that $\vec{X}_i^{(0)}$ is the uniform distribution over the simplex $\Delta^{|\treeset_i|}$, as well as $\bigL_i^{(0)} = \bigL_i^{(-1)} = \vec{0}$. By construction, for every player $i \in \range{m}$ the vector $\vec{X}_i^{(t)}$ is updated using \eqref{eq:omwu} under the sequence of losses $\bigL^{(1)}, \dots, \bigL^{(T)}$, implying that for each $\tree \in \treeset_i$,
\begin{equation}
    \label{eq:expanded-OMWU}
    \vec{X}_i^{(t_0 + t + 1)}[\tree] = \frac{\exp \mleft\{ \eta \mleft( \bigL_i^{(t_0 - 1)}[\tree] - \sum_{s=0}^t \bigL_i^{(t_0 + s)}[\tree] - \bigL_i^{(t_0 + t)}[\tree] \mright) \mright\} \vec{X}_i^{(t_0)}[\tree]}{\sum_{\tree' \in \treeset_i} \exp \mleft\{\eta \mleft( \bigL_i^{(t_0 - 1)}[\tree'] - \sum_{s=0}^t \bigL_i^{(t_0 + s)}[\tree'] - \bigL_i^{(t_0 + t)}[\tree'] \mright) \mright\} \vec{X}_i^{(t_0)}[\tree']}.
\end{equation}
For notational convenience, we will let $\bar{\bigL}^{(t)}_{i, t_0} = \bigL_i^{(t_0 - 1)} - \sum_{s=0}^{t-1} \bigL_i^{(t_0 + s)} - \bigL_i^{(t_0 + t - 1)}$, for $0 \leq t_0 \leq T$ and $t \geq 0$. Moreover, for a vector $\vec{z} \in \R^{|\treeset_i|}$ we define the following function:
\begin{equation}
    \label{eq:softmax-phi}
    \phi_{t_0, \tree}(\vec{z}) = \frac{\exp\{\vec{z}[\tree]\}}{\sum_{\tree' \in \treeset_i'} \vec{X}_i^{(t_0)}[\tree'] \exp \mleft\{\vec{z}[\tree']\mright\}}.
\end{equation}
Equipped with this notation, we can equivalently write \eqref{eq:expanded-OMWU} as $\vec{X}_{i}^{(t_0 + t)}[\tree] = \vec{X}_{i}^{(t_0)}[\tree] \phi_{t_0, \tree}\mleft( \eta \bar{\bigL}^{(t)}_{i, t_0} \mright)$ for $t \geq 1$. In particular, this implies that for any $i' \in \range{m}$ and $\tree_{i'} \in \treeset_{i'}$,

\begin{equation}
    \label{eq:prod-phi}
    \prod_{i' \in \range{m}} \vec{X}_{i'}^{(t_0 + t)} [\tree_{i'}] = \prod_{i' \in \range{m}} \vec{X}_{i'}^{(t_0)}[\tree_{i'}] \phi_{t_0, \tree_{i'}} \mleft( \eta \bar{\bigL}^{(t)}_{i', t_0} \mright).
\end{equation}

Before we proceed with the analysis, let us introduce the \emph{shift operator}. Specifically, for a sequence of vectors $\vec{z} = (\vec{z}^{(1)}, \dots, \vec{z}^{(T)})$, the s-shifted sequence, denoted with $E_s \vec{z}$, is such that $(E_s \vec{z})^{(t)} = \vec{z}^{(t + s)}$, for $1 \leq t \leq T - s$. With this notation, we observe that
\begin{equation*}
    \mleft( D_1 \bar{\bigL}_{i, t_0} \mright)^{(t)} = \bigL_i^{(t_0 + t - 1)} - 2 \bigL_i^{(t_0 + t)} = \bigL_i^{(t_0 + t - 1)} - 2 (E_1 \bigL_i)^{(t_0 + t - 1)},
\end{equation*}
which in particular implies that for any $h' \geq 1$,
\begin{equation}
    \label{eq:shift-recurs}
    \mleft( D_{h'} \bar{\bigL}_{i, t_0} \mright)^{(t)} = (D_{h'-1} \bigL_i)^{(t_0 + t - 1)} - 2 (E_1 D_{h'-1} \bigL_i)^{(t_0 + t - 1)}.
\end{equation}

Next we proceed with bounding $\bar{\bigL}_{i, t_0}^{(t)}$, for any $0 \leq t_0 \leq T$ and $t \geq 0$. In particular, for a fixed $\tree \in \treeset_i$, we know that $\bigL_i^{(t)}[\tree] = \sum_{(j, k) \in E(\tree)} \vec{x}^{(t)}[j] (\vec{\ell}^{(t)}[k] - \vec{\ell}^{(t)}[j])$. Thus, given that $\vec{\ell}_i^{(t)}[j] \in [0, 1]$, for any $j \in \range{n_i}$ and $t \geq 0$, as follows from \eqref{eq:utility-game}, we can conclude that there exists $\tree \in \treeset_i$ such that 
\begin{equation}
    \label{eq:bigL-infty}
    \| \bigL_i^{(t)}\|_{\infty} = \left\lvert \sum_{(j, k) \in E(\tree)} \vec{x}^{(t)}[j](\vec{\ell}^{(t)}[k] - \vec{\ell}^{(t)}[j]) \right\rvert \leq \sum_{(j, k) \in E(\tree)} \vec{x}^{(t)}[j] \left\lvert \vec{\ell}^{(t)}[k] - \vec{\ell}^{(t)}[j] \right\rvert \leq 1,
\end{equation}
where we used that $\left\lvert \vec{\ell}^{(t)}[k] - \vec{\ell}^{(t)}[j] \right\rvert \leq 1$, as well as the fact that $\tree$ is a directed tree, implying that every node has at most one outgoing (directed) edge (see \cref{definition:directed_tree}). Along with the triangle inequality, this implies that 
\begin{equation}
    \label{eq:L-bar-infty}
    \| \bar{\bigL}_{i, t_0}^{(t)} \|_{\infty} = \mleft\| \bigL_i^{(t_0 - 1)} - \sum_{s=0}^{t-1} \bigL_i^{(t_0 + s)} - \bigL_i^{(t_0 + t - 1)} \mright\|_{\infty} \leq (t+2).
\end{equation}
Before we proceed with the next claim, it will be useful to introduce the sequence $\mathfrak{L}^{(t)}$, defined as
\begin{equation*}
    \mathfrak{L}^{(t)} \coloneqq \mleft( \eta \bar{\bigL}_{1, t_0}^{(t)}, \eta \bar{\bigL}_{2, t_0}^{(t)}, \dots, \eta \bar{\bigL}_{m, t_0}^{(t)} \mright).
\end{equation*}

\begin{claim}
    \label{claim:D_h-bound}
Consider some parameter $\alpha \in (0, 1)$ such that $\mleft\| \mleft( D_{h'} \mleft( \eta \bar{\bigL}_{i, t_0} \mright) \mright)^{(t)} \mright\|_{\infty} \leq \frac{1}{B_1} \alpha^{h'} (h')^{B_0 h'}$, for all $i \in \range{m}$, $0 \leq h' \leq h$, and $t \in \range{h + 1 - h'}$, where $B_1 = 12 e^5 m$ and $B_0 \geq 3$. Then, for any $0 \leq t_0 \in T - h - 1$ and $\tree_1 \in \treeset_1, \dots, \tree_m \in \treeset_m$, it holds that
\begin{equation}
    \left\lvert \mleft( D_h \mleft( \prod_{i' \in \range{m}} \vec{X}_{i'}[\tree_{i'}] \mright) \mright)^{(t_0 + 1)} \right\rvert \leq \alpha^h h^{B_0 h + 1} \prod_{i' \in \range{m}} \vec{X}_{i'}^{(t_0)}(\tree_{i'}).
\end{equation}
\end{claim}
\begin{proof}
We will apply \cref{lemma:boundedness-chain-rule} with $n \coloneqq \sum_{i' \in \range{m}} |\treeset_{i'}|$, time horizon $h + 1$, the sequence $\mathfrak{L}^{(t)}$, and the function $\phi$ that maps the concatenation of $\vec{z}_{i'} \in \R^{|\treeset_{i'}|}$, for all $i' \in \range{m}$, to the function $\prod_{i'} \phi_{t_0, \tree_{i'}}(\vec{z}_{i'})$, where $\phi_{t_0, \tree_{i'}}$ was defined in \eqref{eq:softmax-phi}; that is, 
\begin{equation}
    \label{eq:def-phi}
    \phi_{t_0}(\vec{z}_1, \dots, \vec{z}_m) \coloneqq \prod_{i' \in \range{m}} \phi_{t_0, \tree_{i'}}(\vec{z}_{i'}).
\end{equation}
In this context, let us verify the conditions of \cref{lemma:boundedness-chain-rule}. First, \cite[Lemma B.6]{Daskalakis21:Near} implies that the function $\phi_{t_0}$ is $(1, e^3m)$-bounded (in the sense of \cref{lemma:boundedness-chain-rule}), and $B_1 = 12 e^5 m \geq 2e^2 (e^3 m)$. Moreover, by \cite[Lemma B.7]{Daskalakis21:Near} we know that each function $\phi_{t_0, \tree_{i'}}$ has radius of convergence---with respect to the origin $\vec{0}$---at least $1$, and hence, the radius of convergence of $\phi_{t_0}$ is also at least $1$. We also know, by assumption, that $\mleft\| \mleft( D_{h'} \mathfrak{L} \mright)^{(t)} \mright\|_{\infty} \leq \frac{1}{B_1} \alpha^{h'} (h')^{B_0 h'}$, for all $0 \leq h' \leq h$ and $t \in \range{h + 1 - h'}$. As a result, \cref{lemma:boundedness-chain-rule} implies that 
\begin{equation}
    \label{eq:applylemma}
    \left\lvert\mleft(  D_h \mleft( \phi \circ \mathfrak{L} \mright) \mright)^{(1)} \right\rvert \leq \frac{12 e^5 m}{B_1} \alpha^h h^{B_0 h + 1}.
\end{equation}
Finally, we have that 
\begin{align}
    \frac{1}{\prod_{i' \in \range{m}} \vec{X}^{(t_0)}_{i'}[\tree_{i'}] } \left\lvert \mleft( D_h \mleft( \prod_{i' \in \range{m}} \vec{X}_{i'}[\tree_{i'}] \mright) \mright)^{(t_0 + 1)} \right\rvert &= \left\lvert \mleft( D_h \mleft( \prod_{i' \in \range{m}} \mleft( \phi_{t_0, \tree_{i'}} \circ \mleft( \eta \bar{\bigL}_{i', t_0} \mright) \mright) \mright) \mright)^{(1)} \right\rvert \label{eq:align-def-phi} \\
    &= \left\lvert \mleft( D_h \mleft(\phi_{t_0} \circ \mleft( \eta \bar{\bigL}_{1, t_0}, \dots, \eta \bar{\bigL}_{m, t_0} \mright) \mright) \mright)^{(1)} \right\rvert \label{eq:bound_lemma} \\
    &= \left\lvert D_h \mleft( \phi_{t_0} \circ \mathfrak{L} \mright)^{(1)} \right\rvert \notag \\
    & \leq \frac{12 e^5 m}{B_1} \alpha^h h^{B_0 h + 1} = \alpha^h h^{B_0 h + 1} \label{eq:end_bound-frac},
\end{align}
where \eqref{eq:align-def-phi} follows from \cref{eq:prod-phi}; \eqref{eq:bound_lemma} simply uses the definition of $\phi_{t_0}$ in \eqref{eq:def-phi}; and \eqref{eq:end_bound-frac} follows from \eqref{eq:applylemma} (which in turn is a consequence of \cref{lemma:boundedness-chain-rule}), as well as the fact that $B_1 = 12 e^5 m$. This completes the proof.
\end{proof}

\begin{claim}
    \label{claim:inductive_step}
Fix some $1 \leq h \leq H$, a parameter $\alpha \in (0, 1)$, and assume that the learning rate $\eta$ is such that $\eta \leq \min \mleft\{ \frac{\alpha}{36 e^5 m}, \frac{1}{12e^5 (H+3) m} \mright\}$. Moreover, assume that for all $0 \leq h' < h$, $t \leq T - h'$, and $i \in \range{m}$, it holds that $\| (D_{h'} \bigL_i)^{(t)}\|_{\infty} \leq \alpha^{h'} (h' + 1)^{B_0(h' + 1)}$. Then, for all $t \in \range{T - h}$ and $i \in \range{m}$,
\begin{equation}
    \mleft\| \mleft( D_h  \bigL_{i} \mright)^{(t)} \mright\|_{\infty} \leq \alpha^{h} h^{B_0 h + 1}.
\end{equation}
\end{claim}

\begin{proof}
Let us set $B_1 \coloneqq 12 e^5 m$, so that $\eta \leq \min \mleft\{ \frac{\alpha}{3 B_1}, \frac{1}{B_1(H+3)} \mright\}$. We know from \eqref{eq:L-bar-infty} that for $t + 2 \leq h + 3$ it follows that
\begin{equation}
    \label{eq:base}
    \mleft\| D_0 \mleft( \eta \bar{\bigL}_{i, t_0} \mright)^{(t)}\mright\|_{\infty} = \eta \mleft\| \bar{\bigL}_{i, t_0}^{(t)} \mright\| \leq \eta (t+2) \leq \frac{1}{B_1},
\end{equation}
where we used the fact that $\eta \leq 1/(B_1(H+3))$. Next, for $1 \leq h' \leq h$,
\begin{align}
    \mleft\| \mleft( D_{h'} \mleft( \eta \bar{\bigL}_{i, t_0} \mright) \mright)^{(t)} \mright\|_{\infty} &\leq \eta \mleft\| \mleft( D_{h' - 1} \bigL_i \mright)^{(t_0 + t - 1)} \mright\|_{\infty} + 2 \eta \mleft\| \mleft( D_{h' - 1} \bigL_i \mright)^{(t_0 + t)} \mright\|_{\infty} \label{eq:align-trian-shift} \\
    &\leq 3 \eta \alpha^{h' - 1} (h')^{B_0 h'} \label{eq:inductive-hypothesis} \\
    &\leq \frac{1}{B_1} \alpha^{h'} (h')^{B_0 h'}, \label{eq:align-small-eta}
\end{align}
where \eqref{eq:align-trian-shift} follows from \eqref{eq:shift-recurs} and the triangle inequality; \eqref{eq:inductive-hypothesis} is a consequence of the assumption in the claim; and \eqref{eq:align-small-eta} uses the fact that $\eta \leq \frac{\alpha}{3 B_1}$. Next, given that $\bigL^{(t)}_i[\tree] = \sum_{(j, k) \in E(\tree)} \vec{x}_i^{(t)}[j] (\vec{\ell}_i^{(t)}[k] - \vec{\ell}_i^{(t)}[j])$, where recall the expression of $\vec{\ell}_i^{(t)}$ in \eqref{eq:utility-game}, we can infer that 
\begin{align}
    \bigL_i^{(t)} &= \sum_{a_{i'} \in \range{n_{i'}}} \hat{\Lambda}(a_1, \dots, a_m) \prod_{i' \in \range{m}} \vec{x}_{i'}[a_{i'}] \notag \\
    &= \sum_{\tree_{i'} \in \treeset_{i'}} \Tilde{\Lambda}(\tree_1, \dots, \tree_m) \prod_{i' \in \range{m}} \vec{X}_{i'}[\tree_{i'}], \label{eq:utility-bigL}
\end{align}
where $\hat{\Lambda}$ and $\Tilde{\Lambda}$ are functions such that $\hat{\Lambda}(\cdot) \in [-1, 1]$ and $\Tilde{\Lambda}(\cdot) \in [-1, 1]$. More precisely, \eqref{eq:utility-bigL} is obtained from \cref{theorem:equivalence}. As a result, similarly to \eqref{eq:bound-Li} we may conclude that 
\begin{equation}
    \left\lvert (D_h \bigL_i)^{(t)}[\tree] \right\rvert \leq  \sum_{\tree_{i'} \in \treeset_{i'}} \left\lvert \mleft( D_h \mleft( \prod_{i' \in \range{m}} \vec{X}_{i'}[\tree_{i'}] \mright) \mright)^{(t)} \right\rvert.
\end{equation}

The next step is to invoke \cref{claim:D_h-bound} in order to bound the induced term. Specifically, by \eqref{eq:base} and \eqref{eq:align-small-eta} we see that its conditions are met, from which we can conclude that for $t \in \range{T - h}$
\begin{align}
    \mleft\| \mleft( D_h \bigL_i \mright)^{(t)} \mright\|_{\infty} &\leq \sum_{\tree_{i'} \in \treeset_{i'}} \left\lvert \mleft( D_h \mleft( \prod_{i' \in \range{m}} \vec{X}_{i'}[\tree_{i'}] \mright) \mright)^{(t)} \right\rvert \label{eq:util-bigL} \\
    &\leq \alpha^h h^{B_0 h + 1} \sum_{\tree_{i'} \in \treeset_{i'}} \prod_{i' \in \range{m}} \vec{X}^{(t-1)}_{i'}[\tree_{i'}] \label{align-cor-lemma} \\
    &= \alpha^h h^{B_0 h + 1}, \label{eq:align-final-norm}
\end{align}
where \eqref{eq:util-bigL} follows from \eqref{eq:utility-bigL}; \eqref{align-cor-lemma} is an immediate application of \cref{claim:D_h-bound}; and \eqref{eq:align-final-norm} follows from the fact that each $\vec{X}_{i'}$ is a probability distribution over the space of directed trees $\treeset_{i'}$, for all $i' \in \range{m}$, and as such the induced product distribution normalizes to $1$.
\end{proof}
Finally, it follows from \eqref{eq:bigL-infty} that $\mleft\| \mleft( D_0 \bigL_i \mright)^{(t)} \mright\|_{\infty} \leq 1 = \alpha^0 1^{B_0 1}$, for all $i \in \range{m}$. Thus, we can inductively invoke \cref{claim:inductive_step} for $B_0 = 3$ to infer that for all $0 \leq h \leq H$, $i \in \range{m}$, and $t \in \range{T - h}$ that $\mleft\| \mleft( D_h \bigL_i \mright)^{(t)} \mright\|_{\infty} \leq \alpha^h h^{3h + 1}$, as long as $\eta \leq \frac{\alpha}{36 e^5 m}$ and $\alpha \leq 1/(H + 3)$. Finally, following the argument given in the proof of \cref{claim:inductive_step}, we obtain that for any $0 \leq h' \leq h$,
\begin{equation*}
    \mleft\| \mleft( D_{h'} \mleft( \eta \bar{\bigL}_{i, t_0} \mright) \mright)^{(t)} \mright\|_{\infty} \leq \frac{1}{B_1} \alpha^{h'} (h')^{3 h'}.
\end{equation*}
Thus, we can invoke \cref{claim:D_h-bound} to conclude that for any $0 \leq t_0 \leq T - h - 1$ and $\tree_{1} \in \treeset_{1}, \dots, \tree_m \in \treeset_{m}$,
\begin{equation*}
    \left\lvert \mleft( D_h \mleft( \prod_{i' \in \range{m}} \vec{X}_{i'}[\tree_{i'}] \mright) \mright)^{(t_0 + 1)} \right\rvert \leq \alpha^h h^{3 h + 1} \prod_{i' \in \range{m}} \vec{X}_{i'}^{(t_0)}(\tree_{i'}).
\end{equation*}
As a result, plugging-in this bound into \eqref{eq:bound-Li} we obtain that for $t \in \range{T - h}$,
\begin{align*}
    \mleft\| \mleft( D_h \vec{L}_i \mright)^{(t)} \mright\|_{\infty} &\leq \sum_{\tree_{i'} \in \treeset_{i'}} \left\lvert \mleft( D_h \mleft( \prod_{i' \in \range{m}} \vec{X}_{i'}[\tree_{i'}] \mright) \mright)^{(t)} \right\rvert \\
    &\leq \alpha^h h^{3 h + 1} \sum_{\tree_{i'} \in \treeset_{i'}} \prod_{i' \in \range{m}} \vec{X}^{(t-1)}_{i'}[\tree_{i'}], \\
    &= \alpha^h h^{3 h + 1},
\end{align*}
completing the proof.
\end{proof}

Finally, we present the proof of \cref{lemma:bound-variance}. The statement of the lemma is recalled below for convenience.

\backind*

\begin{proof}
In correspondence to the statement of \cref{lemma:closeness}, let $C_0 = 1290$ and $C_1 = 8256$. Moreover, let $\alpha = 1/(4H)$ and $\alpha_0 = \sqrt{\alpha/8}/H^3 < 1/(H+3)$. Note that as long as $C \geq 4^4 \cdot 7 \cdot C_1$, it holds that $\eta \leq \min \mleft\{ \frac{\alpha^4}{7C_1}, \frac{\alpha_0}{36e^5 m} \mright\}$. \cref{lemma:high-order-smooth} implies that for all $i \in \range{m}$, $0 \leq h \leq H$, and $1 \leq t \leq T - h$, it holds that 
\begin{equation*}
    %\label{eq:high-order-smooth}
    \mleft\| \mleft( D_h \vec{L}_i \mright)^{(t)} \mright\|_{\infty} \leq h \mleft(\alpha_0 h^3 \mright)^{h} \leq H \mleft( \alpha_0 H^3 \mright)^h.
\end{equation*}
In particular, along with \cref{claim:var-infty} this implies that 
\begin{align}
    \sum_{t=1}^{T - H} \var_{\vec{p}_i^{(t)}} \mleft( \mleft( D_H \vec{L}_i \mright)^{(t)} \mright) &\le \sum_{t=1}^{T-H} \mleft\| \mleft( D_H \vec{L}_i \mright)^{(t)} \mright\|_\infty^2 \nonumber\\
    &\le H^2 (\alpha_0 H^3)^{2H} \,T \nonumber\\
    &\leq 
    \alpha \sum_{t=1}^{T - H + 1} \var_{\vec{p}_i^{(t)}} \mleft( \mleft( D_{H-1} \vec{L}_i \mright)^{(t)} \mright) + H^2 \mleft( \alpha_0 H^3 \mright)^{2H} T.    \label{eq:var-base}
\end{align}
Next, it will be shown via reverse induction that for all $i \in \range{m}$ and $0 \leq h \leq H-1$ it holds that 
\begin{equation}
    \label{eq:inv-induction}
    \sum_{t=1}^{T - h - 1} \var_{\vec{p}_i^{(t)}} \mleft( \mleft( D_{h+1} \vec{L}_i \mright)^{(t)} \mright) \leq \alpha (1 + 2 \alpha)^{H - h - 1} \sum_{t=1}^{T - h} \var_{\vec{p}_i^{(t)}} \mleft( \mleft( D_{h} \vec{L}_i \mright)^{(t)} \mright) + \frac{2 C_0 H^2 \mleft( 2 \alpha_0 H^3 \mright)^{2h}}{\alpha^3}.
\end{equation}
Indeed, the base case $h = H - 1$ can be verified from \eqref{eq:var-base} using that $2^{2(H-1)} \geq 2^H \geq T$, for $H \geq 2$ and $H = \lceil \log T \rceil \geq \log T$, as well as the fact that 
\begin{equation*}
    1 \leq \frac{2 C_0}{\alpha^3 \mleft( \alpha_0 H^3 \mright)^2} = \frac{2 C_0}{\alpha^4/8} \iff C_0 \geq \frac{\alpha^4}{16}, 
\end{equation*}
since $\alpha = 1/(4H) \leq 1/8$. Next, assume that \eqref{eq:inv-induction} holds for some $1 \leq h \leq H - 1$. We will show the claim for $h - 1$. In particular, we start with the following observation:
\begin{claim}[Multiplicative Stability of (O)MWU]
    \label{claim:mult-stabl}
    For every player $i \in \range{m}$ the sequence $\vec{p}_i^{(1)}, \dots, \vec{p}_i^{(T)}$ is $7\eta$-multiplicatively close.
\end{claim}
\begin{proof}
We know from the update rule of \eqref{eq:omwu} that 
\begin{equation*}
    \vec{p}_i^{(t+1)}[\edge{j}{k}] = \frac{\exp\{- \eta (2 \vec{L}_i^{(t)}[\edge{j}{k}] - \vec{L}_i^{(t-1)}[\edge{j}{k}] )\}}{\sum_{a \neq b} \exp\{ - \eta (2 \vec{L}_i^{(t)}[\edge{a}{b}] - \vec{L}_i^{(t-1)}[\edge{a}{b}])\} \vec{p}_i^{(t)}[\edge{a}{b}]} \vec{p}_i^{(t)}[\edge{j}{k}].
\end{equation*}
Thus, since $\| \vec{L}_i^{(t)} \|_{\infty} \leq 1$, it follows that 
\begin{align*}
    \vec{p}_i^{(t+1)}[\edge{j}{k}] \leq \frac{\exp\{3 \eta\}}{\sum_{a \neq b} \exp\{ - 3\eta  \} \vec{p}_i^{(t)}[\edge{a}{b}]} \vec{p}_i^{(t)}[\edge{j}{k}] &= \exp \{ 6 \eta \} \vec{p}_i^{(t)}[\edge{j}{k}],
\end{align*}
and similar reasoning yields that $\vec{p}_i^{(t+1)}[\edge{j}{k}] \geq \exp \{ - 6 \eta \} \vec{p}_i^{(t)}[j \to k]$. Finally, the claim follows given that $\exp \{ 6 \eta\} \leq 1 + 7 \eta$ for the $\eta$ considered in the lemma.
\end{proof}
Moreover, for $\zeta = 7 \eta$ and given the choices of $\eta$ and $\alpha$, it follows that $1/(2(T - h + 1)) \leq \zeta \leq \alpha^4/C_1$, verifying the first condition of \cref{lemma:closeness} with respect to the sequences $\vec{q} = (\vec{p}_i^{(1)}, \dots, \vec{p}_i^{(T - h + 1)})$ and $\vec{z} = ((D_{h-1} \vec{L}_i)^{(1)}, \dots, D_{h-1} \vec{L}_i)^{(T - h + 1)})$. In addition, for $M = H (2\alpha_0 H^3)^{h-1}$ and $\mu = \frac{2C_0 H^2 (2\alpha H^3)^{2h}}{\alpha^3}$, the inductive hypothesis \eqref{eq:inv-induction} implies that the second condition of \cref{lemma:closeness} also holds. Thus, an application of \cref{lemma:closeness} and simple algebraic calculations complete the proof of the inductive step. In particular, this implies that \eqref{eq:inv-induction} holds for $h = 0$. As a result, given that (by the triangle inequality) $\| \vec{L}_i^{(t)} - \vec{L}_i^{(t-1)}\|_{\infty} \leq 2$, we may conclude that 
\begin{align}
    \sum_{t=1}^T \var_{\vec{p}_i^{(t)}} \mleft( \vec{L}_i^{(t)} - \vec{L}_i^{(t-1)} \mright) &\leq 4 + \sum_{t=2}^T \var_{\vec{p}_i^{(t)}} \mleft( \vec{L}_i^{(t)} - \vec{L}_i^{(t-1)} \mright) \label{eq:claim:infty} \\
    &\leq 4 + (1 + 7 \eta) \sum_{t=2}^T \var_{\vec{p}_i^{(t)}} \mleft( \mleft( D_1 \vec{L}_i \mright)^{(t)} \mright) \label{eq:align-mul-stab1} \\
    &\leq 4 + (1 + 7 \eta) \mleft( \alpha (1 + 2 \alpha)^{H - 1} \sum_{t=1}^T \var_{\vec{p}_i^{(t)}} \mleft( \vec{L}_i^{(t)} \mright) + \frac{2C_0 H^2}{\alpha^3} \mright) \label{eq:h=0} \\
    &\leq 5 + (1 + 7 \eta) \mleft( \alpha (1 + 2 \alpha)^{H - 1} (1 + 7 \eta) \sum_{t=2}^T \var_{\vec{p}_i^{(t)}} \mleft( \vec{L}_i^{(t-1)} \mright) + \frac{2C_0 H^2}{\alpha^3} \mright) \label{eq:cal-1} \\
    &\leq \alpha (1 + 2\alpha)^H \sum_{t=1}^T \var_{\vec{p}_i^{(t)}} \mleft( \vec{L}_i^{(t-1)} \mright) + \frac{2(1 + 7 \eta) C_0 H^2}{\alpha^3} + 5 \label{eq:cal-2} \\
    &\leq 2 \alpha \sum_{t=1}^T \var_{\vec{p}_i^{(t)}} \mleft( \vec{L}_i^{(t-1)} \mright) + \frac{2 (1 + 7\eta) C_0 H^2}{\alpha^3} + 5, \label{eq:align-mul-stab2}
\end{align}
where \eqref{eq:claim:infty} is an immediate consequence of \cref{claim:var-infty} along with the fact that $\| \vec{L}_i^{(t)} - \vec{L}_i^{(t-1)}\|_{\infty} \leq 2$; \eqref{eq:align-mul-stab1} uses \cref{claim:var-mul}; \eqref{eq:h=0} follows from \eqref{eq:inv-induction} for $h = 0$; \eqref{eq:cal-1} again uses \cref{claim:var-mul} along with the fact that $\alpha (1 + 7 \eta)(1 + 2\alpha)^{H-1} \leq 1$; \eqref{eq:cal-2} follows from the bound $(1 + 7 \eta)^2 \leq (1 + 2 \alpha)$; and finally \eqref{eq:align-mul-stab2} simply uses that $\alpha (1 + 2 \alpha)^H \leq 2 \alpha$ for the choice of $\alpha = 1/(4H)$. This completes the proof of the lemma.
\end{proof}

Finally, we are ready to establish our main theorem, which was summarized in \Cref{theorem:main summary}. Before with proceed with the proof, let us first present the detailed version of the theorem.

\begin{theorem}[Detailed version of \cref{theorem:main summary}]
    \label{thm:main}
Consider a general-sum multi-player game with $m$ agents, with each player $i \in \range{m}$ having $n_i$ actions. If all players select strategies according to algorithm $\slomwu$ with a sufficiently small learning rate $\eta = O\mleft( \frac{1}{m \log^4 T} \mright)$, the internal regret of every player $i \in \range{m}$ is bounded by $O \mleft( m \log n_i \log^4 T \mright)$. Therefore, the average product distribution of play is an $O \mleft( \frac{m \log n_i \log^4 T}{T} \mright)$-approximate correlated equilibrium.
\end{theorem}
\begin{proof}%[Proof of \cref{theorem:main}]
First of all, we know from \cref{theorem:convergence_correlated} that it suffices to show that the internal regret of every player $i \in \range{m}$ is bounded by $O(m \log n_i \log^4 T)$. In particular, by \cref{proposition:internal-external} this reduces to showing that the external regret of the regret minimizer $\mathcal{R}_{\Delta}$ in \cref{algo:irm} operating over the pairs of actions is bounded by $O(m \log n_i \log^4 T)$. But the latter can be easily verified by \cref{lemma:RVU++} and \cref{lemma:bound-variance} (as in the proof of \cite[Theorem 3.1]{Daskalakis21:Near}).
\end{proof}

